Assistive Robot Teleoperation Using Behavior Trees

Robotic assistance in robot arm teleoperation tasks has recently gained a lot of traction in industrial and domestic environment. A wide variety of input devices is used in such setups. Due to the noise in the input signals (e.g., Brain Computer Interface (BCI)) or delays due to environmental conditions (e.g., space robot teleoperation), users need assistive autonomy that keeps them in control while following predefined trajectories and avoids obstacles. This assistance calls for activity representations that are easy to define by the operator and able to take the dynamic world state into consideration. This paper represents Activities of Daily Living using Behavior Trees (BTs) whose inherent readability and modularity enables an end user to define new activities using a simple interface. To achieve this, we augment BTs with Shared Control Action Nodes, which guide the user's input on a trajectory facilitating and ensuring task execution.

==> PHAST BTs/acronyms.tex <==

\begin{acronym}
    \acro{adl}[ADL]{Activity of Daily Living}
    \acroplural{adl}[ADLs]{Activities of Daily Living}
    \acro{sct}[SCT]{Shared Control Template}
    \acroplural{sct}[SCTs]{Shared Control Templates}
    \acro{phast}[PHAST BT]{PHAse Switching Teleoperation Behavior Tree}
    \acroplural{phast}[PHAST BTs]{PHAse Switching Teleoperation Behavior Trees}
    \acro{bt}[BT]{Behavior Tree}
    \acroplural{bt}[BTs]{Behavior Trees}
    \acro{bci}[BCI]{Brain Computer Interface}
    \acro{dof}[DoF]{Degree of Freedom}
    \acroplural{dof}[DoFs]{Degrees of Freedom}
    \acro{lts}[LTS]{Labelled Transition System}
    \acroplural{lts}[LTS]{Labelled Transition Systems}
    \acro{ee}[EE]{End Effector}
    \acro{im}[IM]{Input Mapping}
    \acroplural{im}[IMs]{Input Mappings}
    \acro{ac}[AC]{Active Constraint}
    \acroplural{ac}[ACs]{Active Constraints}
    \acro{scan}[SCAN]{Shared Control Action Node}
    \acroplural{scan}[SCANs]{Shared Control Action Nodes}
    \acro{fsm}[FSM]{Finite State Machine}
    \acroplural{fsm}[FSMs]{Finite State Machines}
    
    \acro{lfd}[LfD]{Learning from Demonstration}
    
\end{acronym}
